$h-p$ spectral element methods for three dimensional elliptic problems on non-smooth domains using parallel computers

Elliptic partial differential equations arise in many fields of science and engineering such as steady state distribution of heat, fluid dynamics, structural/mechanical engineering, aerospace engineering and seismology etc. In three dimensions it is well known that the solutions of elliptic boundary value problems have singular behavior near the corners and edges of the domain. The singularities which arise are known as vertex, edge, and vertex-edge singularities. We propose a nonconforming h-p spectral element method to solve three dimensional elliptic boundary value problems on non-smooth domains to exponential accuracy. To overcome the singularities which arise in the neighbourhoods of the vertices, vertex-edges and edges we use local systems of coordinates. These local coordinates are modified versions of spherical and cylindrical coordinate systems in their respective neighbourhoods. Away from these neighbourhoods standard Cartesian coordinates are used. In each of these neighbourhoods we use a geometrical mesh which becomes finer near the corners and edges. We then derive differentiability estimates in these new set of variables and a stability estimate on which our method is based for a non-conforming h-p spectral element method. The Sobolev spaces in vertex-edge and edge neighbourhoods are anisotropic and become singular at the corners and edges. The method is essentially a least-squares collocation} method and a solution can be obtained using Preconditioned Conjugate Gradient Method (PCGM). To solve the minimization problem we need to solve the normal equations for the least-squares problem. The residuals in the normal equations can be obtained without computing and storing mass and stiffness matrices. Computational results for a number of model problems confirm the theoretical estimates obtained for the error and computational complexity.

==> acknow.tex <==
%\centerline{\huge\bf Acknowledgment}
%\vskip 0.5in
\noindent
First and foremost, I would like to express my deepest gratitude, regards and thanks to my
supervisor Prof. Pravir Dutt for his support, ideas and encouragement throughout my work on
this thesis. His mathematical expertise, excellent guidance, availability and wisdom proved
very stimulating and helpful. I profoundly thank and express deep regards to my co-advisor Dr.
A. S. Vasudeva Murthy for his discussions, invaluable suggestions, comments, motivation and
help at all the stages of my research period.
%
%It has been a enriching experience to work under my supervisors Prof. Pravir Dutt and
% I express my sincere gratitude, regards and thanks to them
%for their  and generous help
% Without their encouragement and support this thesis would not have
%been possible.
%\newline

I sincerely thank all the faculty members of the Department of Mathematics and Statistics,
in particular, I am grateful to Prof. V. Raghavendra, Prof. Peeyush Chandra, Prof. M.
Kadalbajoo, Prof. D. Bahugana, Prof. B. V. Rathish Kumar and Prof. Prabha Sharma for their
teaching and guidance in completing the academic course work and their advice and cooperation
in many ways.
%\newline

I thank Dr. C. S. Upadhyay (Aerospace Engineering) for his valuable suggestions and help
at various stages. I also thank Dr. V. Eswaran (Mechanical Engineering) for his help and
financial support towards the completion of this work. I greatly acknowledge Dr. Tarek
Mathew for spending his precious time and worthy comments on the thesis work personally
and via long e-mails.
%\newline

Special thanks go to the Department of Mathematics and Statistics IIT Kanpur, for providing
me a healthy and friendly academic environment. Thanks are due to Dr. Pankaj Biswas and Dr.
G. Nagaraju for helping me in developing my parallel codes.
%, from whom I learnt the very
%first lessons of coding.% I acknowledge them
%\newline

I express my gratitude to my undergraduate teachers at Aligarh Muslim University, Prof.
M. Imdad, Prof. Q. H. Ansari, Prof. V. A. Khan and many others for their inspiration,
motivation and teachings in academics and personal life as well.% I also
%express my regards for all my school teachers who encouraged me to do well in future.
%\newline

I am indebted to the CSIR (Council of Scientific and Industrial Research, New Delhi) and
IIT Kanpur for providing me financial support that facilitated the completion of this
dissertation.
%\newline

Above all, I would like to express heart felt and affectionate gratitude to my parents
(late) Mr. Shahid Husain and Mrs. Amina Shahid for their support and blessings. Their love
and blessings have consistently empowered me, which is beyond the scope of any acknowledgement
but I make an effort to express my love and gratitude to them.
%\newline

I am finding myself incapable of expressing my gratitude to my elder brother Mr. Zulfiquar Ali,
sister-in-law Mrs. Shabnam Ali, younger brother Mr. Irshad Ali, sisters and brother-in-laws
for their silent support, inspiration and good wishes. In particular, I gladly acknowledge
eldest brother-in-law Mr. Irshad Husain who supported and encouraged me a lot to carry out
this work. I feel happy to mention little masters Raja, Sana, Ali, Hasan and Rohan with whom
I had a lot of fun filled moments to refresh myself.
%\newline
% I am also grateful to all other relatives,
%whose love and blessings helped me in pursuing this research.
%\newline

%Though my circle of friends is very big and it is difficut to pay my heartiest thanks to
%everyone, yet
I would like to express my thanks to all my friends at IIT Kanpur and especially, to Vivek,
Prashant, Ashisha, Nitin, Mohit, Abbas, Puneet, Sumit, Geatchew, Arabin and Aquil for making
my stay so colorful and enjoyable. I would also like to thank my colleagues (\emph{Late})
Anand, Rajpoot, Lipi, Arbaz, Subhashree and Raheem for their support throughout my research
period. I warmly acknowledge my seniors Dr. Javid Ali, Dr. M. Sajid, Dr. Muslim, Dr. S. Lamba
and Dr. N. Kishore for their help, cooperation and discussions.
%\newline

I am thankful to all my seniors and friends from AMU Aligarh and specially, to Dr. Arshad Khan,
Dr. Nabi Ullah Khan, Dr. Yahya Abbasi, Asif, Habib, Masood, Naushad and Pandit with whom I had
unforgettable, lovely days at AMU. Heartiest thanks to my childhood friend Dr. Faheem for his
wonderful friendship and constant support.
%\newline

Lastly, I am profoundly grateful to my loving wife Vandna Husain for her perennial encouragement,
guidance, patience, help and great understanding all the way. I express all my deepest love and
affection to my junior princes Zinia.
%\newline
\vskip 0.50in
\begin{flushright}
(Akhlaq Husain)
\end{flushright}


==> dedication.tex <==
\vspace*{3.2in}
\begin{center}
   Dedicated to my parents \\
   {\bf \textit{(Late)} Mr. Shahid Husain} \& {\bf Mrs. Amina Shahid}\\
   and to my elder brother\\
   {\bf Mr. Zulfiquar Ali}
  \end{center}

